Unwinding Rotations Improves User Comfort with Immersive Telepresence Robots

We propose unwinding the rotations experienced by the user of an immersive telepresence robot to improve comfort and reduce VR sickness of the user. By immersive telepresence we refer to a situation where a 360\textdegree~camera on top of a mobile robot is streaming video and audio into a head-mounted display worn by a remote user possibly far away. Thus, it enables the user to be present at the robot's location, look around by turning the head and communicate with people near the robot. By unwinding the rotations of the camera frame, the user's viewpoint is not changed when the robot rotates. The user can change her viewpoint only by physically rotating in her local setting; as visual rotation without the corresponding vestibular stimulation is a major source of VR sickness, physical rotation by the user is expected to reduce VR sickness. We implemented unwinding the rotations for a simulated robot traversing a virtual environment and ran a user study (N=34) comparing unwinding rotations to user's viewpoint turning when the robot turns. Our results show that the users found unwound rotations more preferable and comfortable and that it reduced their level of VR sickness. We also present further results about the users' path integration capabilities, viewing directions, and subjective observations of the robot's speed and distances to simulated people and objects.

==> defs.tex <==


%% Use this to make index entries appear in the margin
%\usepackage{showidx}

%\usepackage[dvips,ps2pdf]{hyperref} 
%\usepackage{hyperref} 




%% Turn on/off math bold
\def\mbon{\mathversion{bold}}
\def\mboff{\mathversion{normal}}

%% Continuous-time definitions
\def\tf{{\phi}} %% State transition function

\def\queue{{Q}}

%% Nature actions
\def\nata{{\theta}}
\def\natas{{\Theta}} % All nature actions

\def\Xappr{{\hat{X}}} % Approximate state space
\def\Xfappr{{\tilde{X}}} % Approximate state space

%% Borrowed from Devin Balkcom and Matt Mason (ijrr 02 paper):
\newcommand{\FF}[0]{\ensuremath{\Uparrow}}
\newcommand{\BB}[0]{\ensuremath{\Downarrow}}
\newcommand{\LL}[0]{\ensuremath{\curvearrowleft}}
\newcommand{\RR}[0]{\ensuremath{\curvearrowright}}

\def\graph{{\cal G}}

\def\stages{{\cal K}}

\def\histy{{\tilde{y}}} %% History
\def\histu{{\tilde{u}}} %% History
\def\histv{{\tilde{v}}} %% History
\def\histx{{\tilde{x}}} %% History
\def\histz{{\tilde{z}}} %% History
\def\histp{{\tilde{p}}} %% History
\def\histe{{\tilde{e}}} %% History
\def\histtheta{{\tilde{\theta}}} %% History
\def\histyt{{\tilde{y}_t}} %% History
\def\histut{{\tilde{u}_t}} %% History
\def\histxt{{\tilde{x}_t}} %% History
\def\histthetat{{\tilde{\theta}_t}} %% History
\def\histpsit{{\tilde{\psi}_t}} %% History
\def\hspacey{{\tilde{Y}}} %% History
\def\hspaceu{{\tilde{U}}} %% History
\def\hspacex{{\tilde{X}}} %% History
\def\histpt{{\tilde{p}_t}} %% History
\def\histist{{\tilde \ist}}
\def\histq{{\tilde q}}
\def\histplan{{\tilde\plan}}

%% Information space notation
\def\ic{{\eta_0}} %% Initial condition
\def\ics{{{\cal I}_0}} %% Initial condition space
\def\ici{{\eta^i_0}} %% Initial condition
\def\icsi{{{\cal I}^i_0}} %% Initial condition space
\def\ist{{\eta}} %% Information state
\def\istder{{\eta_{der}}} %% Information state
\def\ifs{{\cal I}} %% An information space
\def\ifsder{{\cal I}_{der}} %% History information space
\def\ifsderp{{\cal I}'_{der}} %% History information space
\def\ifsest{{\cal I}_{est}} %% History information space
\def\ifshist{{\cal I}_{hist}} %% History information space
\def\ifsndet{{\cal I}_{ndet}} %% Nondeterministic information space
\def\ifsprob{{\cal I}_{prob}} %% Probabilistic information space
\def\ifsgauss{{\cal I}_{gauss}} %% Probabilistic information space
\def\ifsapp{{\cal I}_{app}} %% Probabilistic information space
\def\ifsmom{{\cal I}_{mom}} %% Probabilistic information space
\def\ifsk{{{\cal I}_k}} %% Native information space
\def\ifst{{{\cal I}_t}} %% Native information space
\def\imap{{\kappa}}
\def\imapndet{{\imap_{ndet}}}
\def\imapprob{{\imap_{prob}}}
\def\imapstage{{\imap_{stage}}}
\def\imapapp{{\imap_{app}}}
\def\imapmom{{\imap_{mom}}}
\def\imapgauss{{\imap_{mom}}}
\def\imapsf{{\imap_{sf}}}
\def\cifs{\ifs_c} %% Collapsed information space
\def\cist{\eta^c} %% Information space
\def\mifs{{\kappa}}
\def\imifs{{\Gamma^{-1}}}
\def\allp{{\Pi}} %% All plans
\def\allpc{{\Pi_\kappa}} %% All plans
\def\ite{{f_\ifs}} %% Information transition equation
\def\iteder{{f_\ifs}_{der}} %% Information transition equation
\def\hplan{{\cal H}} %% Information space
\def\difs{{\cal I}_\imap} %% Information space

\def\infX{{\vec{X}}}
\def\infx{{\vec{x}}}
\def\infU{{\vec{U}}}
\def\infu{{\vec{u}}}
\def\infTheta{{\vec{\Theta}}}
\def\inftheta{{\vec{\theta}}}
\def\inff{{\vec{f}}}
\def\infL{{\vec{L}}}
\def\infl{{\vec{l}}}


\def\Land{{\cal L}}

\def\ehat{\hat{e}}
\def\Ehat{\hat{E}}

\def\utility{{\cal U}}

% D^* definitions

\def\Gbest{{G_{best}}}
\def\Gcur{{G_{cur}}}
\def\Gvia{{G_{via}}}


%% This can be redef'ed later to be whatever we want for the robot
\def\A{{\cal A}}

%% Homeomorphism
\def\homeo{{ \;\cong\; }}

%%% The configuration space?
%\def\Q{{\cal Q}}

\def\choose#1#2{{(^{#1}_{#2})}}

\def\sgn{{\rm sgn}}
\def\sgnv{{\rm sgn}}

\def\pow{{\rm pow}}

\def\pdf{{p}}

%% closed chains
\def\Cclo{{{\cal C}_{clo}}}
\def\Cfea{{{\cal C}_{fea}}}


%% manip
\def\Csta{{{\cal C}_{sta}}}
\def\Cgr{{{\cal C}_{gr}}}
\def\Ctra{{{\cal C}_{tra}}}
\def\Cadm{{{\cal C}_{adm}}}
\def\Caobs{{{\cal C}^a_{obs}}}
\def\Cpobs{{{\cal C}^p_{obs}}}
\def\Capobs{{{\cal C}^{ap}_{obs}}}
\def\Xsta{{X_{sta}}}
\def\Xgr{{X_{gr}}}
\def\Xtra{{X_{tra}}}
\def\Ccon{{{\cal C}_{con}}}
\def\motcom{{\mu}}
\def\allmotcom{{\cal M}}


%%time var
\def\tva{{\tau}}
\def\tvb{{\sigma}}
\def\tvc{{\phi}}
\def\tvd{{g}}

%% multi
\def\multa{{\tau}}
\def\multb{{h}}
\def\cubesim{{\square}}

%% Conformation stuff
\def\confv{{q}}

%% General transformation
\def\gt{{h}}
\def\gti{{h^{-1}}}

%% Translation parameters
\def\xt{x_t}
\def\yt{y_t}
\def\zt{z_t}

%% Logical predicates
\def\lpred{\phi}
\def\qfpred{\phi}
\def\plpred{\alpha}
\def\quant{{\cal Q}}
\def\tarsk{\Phi}
\def\qftask{\phi}
\def\polys{{\cal F}} % Set of polynomials
\def\proot{{\beta}} % Polynomial root

%% Canny's method
\def\polyf{{\psi}}
\def\cmap{{h}}

%% C-space definitions
\def\C{{\cal C}}
\def\Cobs{{\cal C}_{obs}}
\def\Cfree{{\cal C}_{free}}
\def\CP{{P}}
\def\qinit{{q_{I}}}
\def\qgoal{{q_{G}}}
\def\qcur{{q_{cur}}}
\def\qnew{{q_{new}}}
\def\qiinit{{q^i_{I}}}
\def\qigoal{{q^i_{G}}}
\def\qoneinit{{q^1_{I}}}
\def\qonegoal{{q^1_{G}}}
\def\qminit{{q^m_{I}}}
\def\qmgoal{{q^m_{G}}}

\def\Xobs{{X_{obs}}}
\def\Xfree{{X_{free}}}
\def\Xcon{{X_{con}}}
\def\Xric{{X_{ric}}}
\def\xinit{{x_{I}}}
\def\xgoal{{x_{G}}}
\def\Xgoal{{X_{G}}}
\def\xcur{{x_{cur}}}
\def\xnew{{x_{new}}}

\def\B{{\cal B}}
\def\D{{\cal D}}
\def\I{{\cal I}}
\def\J{{\cal J}}
\def\K{{\cal K}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\N{{\cal N}}
\def\O{{\cal O}}
\def\P{{\cal P}}
\def\U{{\cal U}}
\def\W{{\cal W}}
\def\X{{\cal X}}

\def\Ufree{{\U_{free}}}

% Mapping for a singular simplex
\def\sing{{\sigma}}

\def\x{{ x}}
\def\u{{ u}}

\def\Uf{{\vec U}}
\def\Vf{{\vec V}}
\def\Wf{{\vec W}}
\def\Zf{{\vec Z}}

% Complexes
\def\Comp{{\cal K}}
\def\Cell{C}
\def\Simp{\Delta}

% van der Corput sequence
\def\vdc{{\nu}}
% General sequence
\def\genseq{{\alpha}}

\def\Re{{\mathbb{R}}}
\def\Com{{\mathbb{C}}}
\def\Z{{\mathbb{Z}}}
\def\S{{\mathbb{S}}}
\def\H{{\mathbb{H}}}
\def\Q{{\mathbb{Q}}}
\def\Nat{{\mathbb{N}}}
\def\RP{{\mathbb{RP}}}
\def\F{{\mathbb{F}}}
\def\T{{\mathbb{T}}}
\def\One{{\bf 1_G}}
\def\Ra{{\mathbb{A}}}
\def\Vs{{V}}

\def\Fcal{{\cal F}}

\def\q{{q}}

%% Randomized strategy
\def\urand{{w}}

\def\qq1{{q_1}}
\def\qk{{q_k}}
\def\qi{{q_i}}
\def\qkp1{{q_{k+1}}}
\def\qKp1{{q_{F}}}
\def\qKi{{q_{K+1}}}
\def\qKp1{{q_{F}}}
\def\qi{{q_{F}}}
\def\qxq1{{q_1}}

\def\uu1{{u_1}}
\def\uk{{u_k}}
\def\uK{{u_K}}
\def\ui{{u_i}}
\def\xk{{x_k}}
\def\xi{{x_i}}
\def\xkp1{{x_{k+1}}}
\def\xKp1{{x_{F}}}
\def\xKi{{x_{F}}}
\def\xq1{{x_1}}
\def\ukp1{{u_{k+1}}}
\def\thetak{{\theta_k}}

% These are backward actions
\def\bwactset{{U^{-1}}}
\def\bwact{u^{-1}}
\def\bwf{{f^{-1}}}

\def\octg{G^*}        % Optimal cost to go
\def\octc{C^*}        % Optimal cost to come 
\def\eoctg{G^*}       % expected Optimal cost to go
\def\eoctc{C^*}       % expected Optimal cost to come 
\def\woctg{G^*}       % worst-case Optimal cost to go
\def\wctg{G}       % worst-case cost to go
\def\woctc{C^*}       % worst-case Optimal cost to come 
\def\ctg{{G}}         % Cost-to-go   -- not necessarily optimal
\def\ctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\wctgpl{{G_\plan}}         % Cost-to-go   -- not necessarily optimal
\def\ctc{{C}}         % Cost-to-come -- not necessarily optimal
\def\ectg{\hat{G}^*}  % Estimated cost-to-go (A-star)
\def\ctgs{{g}}         % Cost-to-go for use in sampling chapter -- conflict with G
\def\exctg{G}       % expected Optimal cost to go
\def\exctgpl{G_\plan}       % expected Optimal cost to go
\def\exctc{C}       % expected Optimal cost to come 
\def\eoj{J^*}
\def\eojpl{J_\plan}
\def\qval{Q^*}
\def\aqval{\hat{Q}^*}
\def\qvalpl{Q_\plan}
\def\eectg{\hat{G}_\plan}

\def\cmean{\bar{c}}

\def\topi{{/\sim}} % Topological identification
\def\xb{{x_b}}

\def\Polys{{\cal P}}
\def\Poly{{P}}

%% 2D phase space for trajectory planning
\def\tphase{{S}}

%% Game theory
\def\Pa{{{\rm P}_1}}
\def\Pb{{{\rm P}_2}}
\def\Pc{{{\rm P}_3}}
\def\Pli{{{\rm P}_i}}
\def\Pn{{{\rm P}_n}}
\def\upperv{\overline{L}^*}
\def\lowerv{\underline{L}^*}
\def\ecost{{\bar{L}}}
\def\uppervm{\overline{\cal L}^*}
\def\lowervm{\underline{\cal L}^*}
\def\gamev{L^*}
\def\gameva{{L^*_a}}
\def\gamevb{{L^*_b}}
\def\gamevm{{\cal L}^*}

%% Plan definitions
\def\plan{\pi}
\def\fplan{\pi} %% Feedback
\def\iplan{\pi}
\def\pplan{\sigma} %% Partial plan
\def\planset{{\Pi}}
\def\fplanset{{\Pi}}

\def\argmax{\operatornamewithlimits{argmax}}
\def\argmin{\operatornamewithlimits{argmin}}
\def\Pre{\operatorname{Pre}}
\def\Back{\operatorname{B}}
\def\SB{\operatorname{SB}}
\def\WB{\operatorname{WB}}
\def\Front{\operatorname{Front}}
\def\mymod{\operatorname{mod}}
\def\erf{\operatorname{erf}}
\def\hull{\operatorname{hull}}
\def\Front{\operatorname{Front}}
\def\atan2{\operatorname{atan2}}
\def\intfn{\operatorname{int}}
\def\dspan{\operatorname{span}}
\def\exp{\operatorname{exp}}
\def\adop{\operatorname{Ad}}
\def\clfn{\operatorname{cl}}
\def\Vor{\operatorname{Vor}}

\def\distr{{\triangle}}
\def\tdiff{{\Delta t}}
\def\lie{{\cal L}}
\def\phall{{\cal PH}}

\def\Cinfeq{{{\tilde C}^\infty}}

\def\truesp{\mbox{\sc{true }}}
\def\falsesp{\mbox{\sc{false }}}
\def\true{\mbox{\sc{true}}}
\def\false{\mbox{\sc{false}}}

\def\sccat{\mbox{\sc{cat}}}
\def\scdog{\mbox{\sc{dog}}}
\def\sctree{\mbox{\sc{tree}}}
\def\schouse{\mbox{\sc{house}}}

\def\qdot{{\dot q}}
\def\pdot{{\dot p}}
\def\qddot{{\ddot q}}
\def\qdddot{{q^{(3)}}}
\def\xdot{{\dot x}}
\def\xddot{{\ddot x}}
\def\yddot{{\ddot y}}
\def\ydot{{\dot y}}
\def\zdot{{\dot z}}
\def\xtdot{{{\dot x}_t}}
\def\ytdot{{{\dot y}_t}}
\def\thetadot{{\dot \theta}}
\def\thetaddot{{\ddot \theta}}
\def\adot{{\dot a}}
\def\bdot{{\dot b}}
\def\ceedot{{\dot c}}
\def\deedot{{\dot d}}
\def\fdot{{\dot f}}
\def\rdot{{\dot r}}
\def\sdot{{\dot s}}
\def\sddot{{\ddot s}}
\def\udot{{\dot u}}
\def\vdot{{\dot v}}
\def\wdot{{\dot w}}
\def\omegadot{{\dot \omega}}
\def\sigmadot{{\dot \omega}}
\def\phidot{{\dot \phi}}
\def\psidot{{\dot \psi}}
\def\alphadot{{\dot \alpha}}
\def\betadot{{\dot \beta}}
\def\gammadot{{\dot \gamma}}
\def\lambdadot{{\dot \lambda}}
\def\hdot{{\dot h}}
\def\gdot{{\dot g}}

\def\xtoq{{\kappa}}

\def\ustar{{u^*}}
\def\E{\operatorname{E}} %Expectation: $\E[X]$ (like \Pr)

\theoremstyle{plain}

%{\theorembodyfont{\rmfamily}\newtheorem{formulation}{Formulation}[chapter]}
%{\theorembodyfont{\rmfamily}\newtheorem{example}{Example}[chapter]}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Def}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{scenario}{Scenario}


\def\ds{\displaystyle\strut}
\def\idz{{\hspace{0.25in}}}

\def\disX{{\check X}}
\def\disx{{\check x}}
\def\disu{{\check u}}
\def\disU{{\check U}}
\def\disxgoal{{{\check x}_g}}
\def\disfplan{{\check \fplan}}
\def\disphi{{\check \phi}}

%% Dynamics
\def\force{{F}}
\def\moment{{N}}
\def\com{{p}} % Center of mass
\def\velcom{{\dot p}} % Center of mass
\def\acccom{{\ddot p}} % Center of mass
\def\mass{{m}}
\def\linmom{{D}} % Linear momentum
\def\angmom{{E}} % Angular momentum
\def\dens{{\sigma}}
\def\covfn{{\histx}} % Function for calculus of variations

\newcommand{\R}{{\mathcal R}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

\newcommand{\qed}{\hfill $\blacksquare$ \hfill \\}


